Deniable Encryption in a Quantum World

(Sender-)Deniable encryption provides a very strong privacy guarantee: a sender who is coerced by an attacker into "opening" their ciphertext after-the-fact is able to generate "fake" local random choices that are consistent with any plaintext of their choice. In this work, we study (sender-)deniable encryption in a setting where the encryption procedure is a quantum algorithm, but the ciphertext is classical. We show that quantum computation unlocks a fundamentally stronger form of deniable encryption, which we call perfect unexplainability. The primitive at the heart of unexplainability is a quantum computation for which there is provably no efficient way, such as exhibiting the "history of the computation", to establish that the output was indeed the result of the computation. We give a construction that is secure in the random oracle model, assuming the quantum hardness of LWE. Crucially, this notion implies a form of protection against coercion "before-the-fact", a property that is impossible to achieve classically.

==> commands.tex <==
\newcommand{\etal}{{et al. }}
\usepackage{amsfonts,latexsym,graphicx,amssymb,amsmath,enumitem,physics}
\usepackage{amsthm}
\usepackage{fullpage}
\usepackage{color} % for textcolor
\usepackage{hyperref,cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% General %%%%%%%%%%%%%%%%%%%%%%%%%
\mathchardef\mhyphen="2D
\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\bit}{\{0,1\}}
\newcommand{\seclam}{1^\lambda}
\newcommand{\msk}{\mathsf{msk}}
\newcommand{\key}{\mathsf{key}}
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\vk}{\mathsf{vk}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\ct}{\mathsf{ct}}
\newcommand{\negl}{\mathsf{negl}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\BQP}{\mathsf{BQP}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\from}{\gets}
\newcommand{\prg}{\mathsf{PRG}}
\newcommand{\Rq}{R_q}
\newcommand{\Zq}{\Z_q}
\newcommand{\st}{^*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Sets, brackets shorthand %%%%%%%%%%%%%
\newcommand{\scl}[1]{\set{{#1}_\lambda}_{\lambda \in \N}}
\newcommand{\sck}[1]{\set{{#1}_\kappa}_{\kappa \in \N}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\sset}[1]{\{#1\}}
\newcommand{\brackets}[1]{\ensuremath{\left( #1 \right)}}
\newcommand{\Brackets}[1]{\ensuremath{\left[ #1 \right]}}
\newcommand{\nat}[1]{\ensuremath{\Brackets{1, #1}}}
\newcommand{\natz}[1]{\ensuremath{\set{0, 1, \ldots, #1}}}
\newcommand{\nato}[2]{\ensuremath{\set{#1, \ldots, #2}}}
% \newcommand{\ket}[1]{|#1\rangle}
% \newcommand{\bra}[1]{\langle#1|}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% Calligraphic letters %%%%%%%%%%%%%%%%%
%%% Missing letters F, H, L, N, O, P, Z
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\G}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}
\newcommand{\R}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\T}{\ensuremath{\mathcal{T}}}
\newcommand{\U}{\ensuremath{\mathcal{U}}}
\newcommand{\V}{\ensuremath{\mathcal{V}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}
\newcommand{\X}{\ensuremath{\mathcal{X}}}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}}
\newcommand{\mat}[1]{\mathbf{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% Theorem, lemma, etc %%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}{Claim}[theorem]
\newtheorem{fact}{Fact}[theorem]
\newtheorem{definition}{Definition}[theorem]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}[theorem]
\newtheorem{remark}{Remark}[theorem]
\newtheorem{construction}{Construction}
%\newtheorem{cclaim}{Claim}
% keep the following for lncs
\newtheorem{assumption}{Assumption}
\newtheorem{observation}{Observation}

%%%%%%%%%%% Referring to stuff %%%%%%%%%%% %%%%%%%%%%%%%%
\newcommand{\defref}[1]{Definition~\protect\ref{def:#1}}
\newcommand{\secref}[1]{Section~\protect\ref{sec:#1}}
\newcommand{\appref}[1]{Appendix~\protect\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\protect\ref{fig:#1}}
\newcommand{\tblref}[1]{Table~\protect\ref{tbl:#1}}
\newcommand{\tableref}[1]{Table~\protect\ref{table:#1}}

\newcommand{\thmref}[1]{Theorem~\protect\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\protect\ref{lem:#1}}
\newcommand{\obsref}[1]{Observation~\protect\ref{obs:#1}}
\newcommand{\clmref}[1]{Claim~\protect\ref{clm:#1}}
\newcommand{\claimref}[1]{Claim~\protect\ref{claim:#1}}
\newcommand{\assref}[1]{Assumption~\protect\ref{ass:#1}}

\newcommand{\corref}[1]{Corollary~\protect\ref{cor:#1}}
\newcommand{\fctref}[1]{Fact~\protect\ref{fct:#1}}
\newcommand{\eqnref}[1]{Equation~(\protect\ref{eqn:#1})}
\newcommand{\rmkref}[1]{Remark~\protect\ref{rmk:#1}}
\newcommand{\asmref}[1]{Assumption~\protect\ref{asm:#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Protocols, figures %%%%%%%%%%
\renewcommand{\figurename}{Protocol}

\newlength{\protowidth}
\newcommand{\pprotocol}[5]{
{\begin{figure*}[#4]
\begin{center}
\setlength{\protowidth}{\textwidth}

%\addtolength{\protowidth}{-3\intextsep}

% \fbox{
%         \small
%         \hbox{\quad
%         \begin{minipage}{\protowidth}
%         \begin{center}
%         {\bf #1}
%         \end{center}
%         #5
%         \end{minipage}
%         \quad}
%         }
        {
        \hrulefill \vspace{5pt}
        \small
        {\quad
        \begin{minipage}{\protowidth}
        \begin{center}
        {\bf #1}
        \end{center}
        #5

        \hrulefill

        \end{minipage}
        \quad}
        }

        \caption{\label{#3} #2}
\end{center}
\vspace{-4ex}
\end{figure*}
} }


\newcommand{\protocol}[4]{
\pprotocol{#1}{#2}{#3}{tbh!}{#4} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%% prelims %%%%%%%%%%
\newcommand{\rlweqchi}{\mathsf{RLWE}_{R, q,\chi}}
\newcommand{\Rn}{R_n}
\newcommand{\Rnqn}{R_{n, q_n}}
\newcommand{\Rnq}{R_{n,q}}
\newcommand{\Rqn}{R_{n,q}}
\newcommand{\gentrap}{\textsc{GenTrap}}
\newcommand{\inv}{\textsc{Invert}}
\newcommand{\rhoXE}{\rho_{XE}}
\newcommand{\rhoxE}{\rho^x_E}
\newcommand{\pguess}{p_{\mathrm{guess}}}
\newcommand{\minent}{{H_{\infty}}}
\newcommand{\dm}{\mathsf{D}}
\newcommand{\dg}{\dagger}
\newcommand{\Id}{\mathsf{Id}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% NTCFs %%%%%%%%%%
\newcommand{\trap}{\tau}
\newcommand{\trapf}{\kappa}
\newcommand{\supp}{\textsc{Supp}}
\newcommand{\genf}{\textsc{Gen}_{\mathcal{F}}}
\newcommand{\invf}{\textsc{Inv}_{\mathcal{F}}}
\newcommand{\chkf}{\textsc{Chk}_{\mathcal{F}}}
\newcommand{\sampf}{\textsc{Samp}_{\mathcal{F}}}
\newcommand{\J}{\mathsf{BitDecomp}}
\newcommand{\bdx}{\overline{x}}
\newcommand{\hatg}[1]{\hat{G}_{{#1}}}
\newcommand{\Es}[1]{E_{#1}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mata}{\vec{a}}
\newcommand{\mate}{\vec{e}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Quantum supremacy %%%%%%%%%%
\newcommand{\cnt}{\mathsf{count}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% randomness %%%%%%%%%%
\newcommand{\hash}{H}
\newcommand{\PHkymd}{\mathsf{P}_{k,\hash}^{y,m,d}}
\newcommand{\BHky}{\mathsf{B}_{k,\hash}^y}
\newcommand{\phist}{\phi}
\newcommand{\stateone}{\rho}
\newcommand{\comp}[1]{\overline{#1}}
\newcommand{\My}{M_y}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\phione}{\phi_1}
\newcommand{\phitwo}{\phi_2}
\newcommand{\acchk}{\mathsf{Acc}_{\hash,k}}
\newcommand{\prbd}{q}
\newcommand{\query}{Q}
\newcommand{\HfourQ}{\calH_{4 \query}}
\newcommand{\Axh}{\mathsf{A}_{\hash}^{x_0, x_1, h}}
\newcommand{\Bxh}{\mathsf{B}_{\hash}^{x_0, x_1, h}}
\newcommand{\RH}{\R_{\hash}}
